CoronaViz: Visualizing Multilayer Spatiotemporal COVID-19 Data with Animated Geocircles

While many dashboards for visualizing COVID-19 data exist, most separate geospatial and temporal data into discrete visualizations or tables. Further, the common use of choropleth maps or space-filling map overlays supports only a single geospatial variable at once, making it difficult to compare the temporal and geospatial trends of multiple, potentially interacting variables, such as active cases, deaths, and vaccinations. We present CoronaViz, a COVID-19 visualization system that conveys multilayer, spatiotemporal data in a single, interactive display. CoronaViz encodes variables with concentric, hollow circles, termed geocircles, allowing multiple variables via color encoding and avoiding occlusion problems. The radii of geocircles relate to the values of the variables they represent via the psychophysically determined Flannery formula. The time dimension of spatiotemporal variables is encoded with sequential rendering. Animation controls allow the user to seek through time manually or to view the pandemic unfolding in accelerated time. An adjustable time window allows aggregation at any granularity, from single days to cumulative values for the entire available range. In addition to describing the CoronaViz system, we report findings from a user study comparing CoronaViz with multi-view dashboards from the New York Times and Johns Hopkins University. While participants preferred using the latter two dashboards to perform queries with only a geospatial component or only a temporal component, participants uniformly preferred CoronaViz for queries with both spatial and temporal components, highlighting the utility of a unified spatiotemporal encoding. CoronaViz is open-source and freely available at http://coronaviz.umiacs.io.

==> scraps.tex <==
We 
Some like 
the number of confirmed cases and deaths are also reported as a result of
normalization with respect to a measure such as per 100,000
inhabitants (termed an incidence rate). Others like the number of
deaths are  normalized with respect to the number of confirmed cases
(termed a mortality rate). The visualization enables spatial and 
temporal variation.


\begin{figure}
    \centering
    \subfloat[Log scale (base 10).]{
        \includegraphics[width=0.33\textwidth,trim=0cm 3cm 0cm 2cm,clip]{log10.png}
        \label{fig:log10}
    }\\
    \subfloat[Log scale (base $e$).]{
        \includegraphics[width=0.33\textwidth,trim=0cm 3cm 0cm 2cm,clip]{ln.png}
        \label{fig:ln}
    }
    \caption{Log scale.}
    \label{fig:log-base}
\end{figure}

\begin{figure*}[tbh]
    \centering
    \subfloat[U.S. cases in the April window.]{
        \includegraphics[width=0.45\textwidth,trim=0cm 3cm 0cm 0.8cm,clip]{april-us-states.png}
        \label{fig:us-april}
    }
    \subfloat[U.S. cases in the July window.]{
        \includegraphics[width=0.45\textwidth,trim=0cm 3cm 0cm 0.8cm,clip]{figures/july-us-states.png}
        \label{fig:us-july}
    }\\
    \subfloat[U.S. cases in the September window.]{
        \includegraphics[width=0.45\textwidth,trim=0cm 3cm 0cm 0.8cm,clip]{sept-us-states.png}
        \label{fig:us-sept}
    }
    \subfloat[Charts from the \textit{Washington Post}.]{
        \includegraphics[width=0.45\textwidth,trim=0cm 5cm 0cm 0.8cm,clip]{washington-post.png}
        \label{fig:washingtonpost}
    }
    \caption{CoronaViz map vs.\ \textit{Washington Post} charts~(\href{https://www.youtube.com/watch?v=UcDjFLa3I_Y}{\color{blue}\underline{video}})}
    \label{fig:coronaviz-vs-washingtonpost}
\end{figure*}



==> tvcg-journal-latex-2019.10.01/tools-table.tex <==
\begin{table*}[h!]
%\centering
\begin{tabular}{|l l|} 
 \hline
 Col1 & Col2 \\ [0.5ex] 
 \hline
Coronavirus COVID-19 global cases (Johns Hopkins) & \url{https://coronavirus.jhu.edu/} \\
Novel Coronavirus (COVID-19) outbreak timeline map  (HealthMap) & \url{https://www.healthmap.org/ncov2019/} \\
(Google News) & \url{https://news.google.com/covid19/map} \\
Novel coronavirus infection map (University of Washington) & \url{https://hgis.uw.edu/virus/} \\
COVID-19 surveillance dashboard (University of Virginia) & \url{http://nssac.bii.virginia.edu/covid-19/dashboard/} \\
Novel coronavirus (COVID-19) situation dashboard (WHO) & \url{https://covid19.who.int/} \\
Coronavirus disease 2019 in the US (CDC) & \url{https://www.cdc.gov/coronavirus/2019-ncov/cases-in-us.html} \\
Geographical distribution of COVID-19 cases worldwide (ECDC) & \url{https://www.ecdc.europa.eu/en/geographical-distribution-2019-ncov-cases} \\
COVID-19 coronavirus tracker (Kaiser Family Foundation) & \url{https://www.kff.org/global-health-policy/fact-sheet/coronavirus-tracker/} \\
COVID-19 coronavirus outbreak (Worldometer) & \url{https://www.worldometers.info/coronavirus/} \\
Coronavirus: the new disease Covid-19 explained (South China Morning Post) & \url{https://multimedia.scmp.com/infographics/news/china/article/3047038/wuhan-virus/index.html} \\
Mapping the Wuhan coronavirus outbreak (ESRI StoryMaps) & \url{https://storymaps.arcgis.com/stories/4fdc0d03d3a34aa485de1fb0d2650ee0} \\
(Flourish) & \url{https://public.flourish.studio/visualisation/1539110} \\
(1point3acres) & \url{https://coronavirus.1point3acres.com/en} \\
(University of Wisconsin) & \url{https://geods.geography.wisc.edu/covid19/physical-distancing/} \\
Regenstrief COVID-19 Dashboard~\cite{dixon2021leveraging} & \url{https://www.regenstrief.org/covid-dashboard/} \\ \hline
\end{tabular}
\caption{Table to test captions and labels.}
\label{tab:tools}
\end{table*}

